Revisiting Ensemble Methods for Stock Trading and Crypto Trading Tasks at ACM ICAIF FinRL Contest 2023-2024

Reinforcement learning has demonstrated great potential for performing financial tasks. However, it faces two major challenges: policy instability and sampling bottlenecks. In this paper, we revisit ensemble methods with massively parallel simulations on graphics processing units (GPUs), significantly enhancing the computational efficiency and robustness of trained models in volatile financial markets. Our approach leverages the parallel processing capability of GPUs to significantly improve the sampling speed for training ensemble models. The ensemble models combine the strengths of component agents to improve the robustness of financial decision-making strategies. We conduct experiments in both stock and cryptocurrency trading tasks to evaluate the effectiveness of our approach. Massively parallel simulation on a single GPU improves the sampling speed by up to $1,746\times$ using $2,048$ parallel environments compared to a single environment. The ensemble models have high cumulative returns and outperform some individual agents, reducing maximum drawdown by up to $4.17\%$ and improving the Sharpe ratio by up to $0.21$. This paper describes trading tasks at ACM ICAIF FinRL Contests in 2023 and 2024.

==> deleted.tex <==
%However, two major challenges—policy instability and sampling bottlenecks—are faced. The challenge of policy instability significantly impacts the performance and reliability of agents in reinforcement learning. Financial markets further complicate the development of stable policies due to their highly complex and dynamic nature ~\cite{liu2024dynamic}. Therefore, in financial reinforcement learning, policies frequently exhibit significant variability, often leading to inconsistent and unreliable performance. To mitigate policy instability associated with a single agent, ensemble methods can be used. Ensemble methods have consistently shown effectiveness in enhancing the robustness of models \cite{yang2020deep}, by aggregating diverse algorithms to combine individual model strengths and mitigate their vulnerabilities ~\cite{ensemble_ganaie}. While the ensemble method mitigates policy instability, the training of multiple agents with extensive financial datasets encounters a sampling bottleneck. The challenge of sampling bottleneck arises from the intensive computational requirements of simulating complex financial markets, where data sampling is an inherently time-consuming process. With the ensemble method, the burden of data sampling scales with the number of component models. Fig. \ref{fig:producer_consumer} (a) shows a traditional training process in the Producer-Consumer framework. The simulation phase, managed by the "Producer" and executed on CPUs, produces the samples. The samples will be stored in a replay buffer. The learning phase, managed by the "Consumer" and typically run on GPUs, fetches the data in the buffer and uses it for policy updating. This process introduces latency over a bidirectional PCIe data transfer, which is required to synchronize the CPU and GPU during training. The sampling process and transferring latency create a significant bottleneck, considerably slowing down training and hindering a seamless integration of the simulation and learning processes. 

%To perform the stock trading task, different agents are trained, including Proximal Policy Optimization (PPO) [XX], Soft Actor-Critic (SAC) [XX], and Deep Deterministic Policy Gradient (DDPG) [XX]. We use historical daily open, high, low, close, and volume (OHLCV) data for 30 stocks in the Dow Jones index between 2020 and 2023. Each type of agent is trained and tested $10$ times.
% We train and test models on a rolling window basis, using $30$ days for testing and $5$ days for trading.
%Their cumulative returns over a test window are shown in Fig. \ref{fig:observation_experiment} (a)-(c), with a solid line representing average performance. The standard deviation of the cumulative returns over $10$ tests was calculated and then averaged over trading dates. Policy instability is evident from the wide shaded areas for each agent that depict the range between the highest and lowest returns. We also conducted the same experiment for an ensemble model with agent action averaging. The ensemble method aggregates PPO, SAC, and DDPG agents, with their different strengths and weaknesses shown in Table \ref{tab:compare_agents}. As shown in Fig. \ref{fig:observation_experiment} (d), the ensemble model has a significantly smaller range of performance differences than those of individual agents. The ensemble model's mean difference between the Max and Min performance is around half of those of individual agents. The average standard performance of returns for the ensemble is $X$ compared with individual agents. This result confirms that ensemble methods can help mitigate policy instability and improve performance by combining the strengths and balancing the weaknesses of individual models. An ensemble of reinforcement learning models can provide a more robust solution in financial markets, where the environment changes rapidly and agent optimality is crucial. 

%Various RL learning algorithms such as actor algorithms, critic algorithms, and actor-critic algorithms exist; due to their ability to perform well in large and complex environments, the actor-critic approach has been gaining traction in the financial space  ~\cite{yang2020deep} ~\cite{liu2021finrl}. 

%RL algorithms rely heavily on simulated environments for training, especially financial algorithms, which need to be trained and verified on historical data before being deployed to real-world applications. To date, market simulation environments leverage CPUs to run the environments, whilst the models are trained on GPUs ~\cite{byrd2020abides}. These pipelines limit the number of environments to the number of CPU cores and introduce latency when information is passed between the CPU and GPU. This is a large bottleneck in financial settings, where data is simple and frequently updated. To address this issue, researchers have developed GPU-based simulation learning environments ~\cite{makoviychuk2021isaac}, which allow both the simulation environment and the learning process to be handled on the GPU, removing the data transfer and the CPU core count bottlenecks. In finance, Sascha Frey et al. developed JAX-LOB, a GPU-accelerated limit order book (LOB) simulator specifically designed to enable the parallel processing of thousands of books on GPUs ~\cite{jaxlob}.


% In Fig. \ref{fig:producer_consumer} (a), the simulation phase is executed on CPUs and the number of samples is limited. To update the policy network on the GPU, the "Consumer" must pass the PCIe to access data on the CPU and then synchronize the updated policy via the PCIe again. This process incurs high communication costs between GPU and CPU and the amount of data sampled is limited. As ensemble methods require training multiple agents, this sampling bottleneck will become a major challenge for training efficiency.

% The sampling bottleneck can be addressed by With the end-to-end data sampling and policy updating directly on GPU. As shown in (b), the simulation phase can produce more samples in the same amount of time on GPU, and the communication costs over PCIe are eliminated. In addition, employing multiple agents trained on GPU enhances the development of an ensemble method, resulting in greater stability.

% As Fig. \ref{fig:producer_consumer} shows, a vectorized environment manages multiple sub-environments to simulate different market scenarios. As shown in Fig \ref{fig:simulation_gpu}, each sub-environment maintains its own market conditions, including balances, prices, holding positions, and technical factors. The GPU hosts many cores that are utilized to execute numerous threads concurrently. In our setup, multiple threads can be responsible for managing the interaction between a sub-environment (SubEnv) and the agent. Among these, each thread performs different simple operations such as updating balances and calculating rewards. The trajectories, consisting of a sequence of states ($s$), actions ($a$), and rewards ($r$), sampled from the interaction between the sub-environments and the agent, are stored as tensors in the GPU memory. We add a new dimension representing the number of environments in the tensors to enhance the organization of parallel simulation. Therefore, $s_t^k$ in the memory represents the state at time $t$ obtained from the environment $k$. The collective samples are crucial for the agent's policy updates and are efficiently handled through the GPU’s high-throughput memory bandwidth.

% \begin{enumerate}
%     \item \textbf{Training}. Each agent is trained independently within its respective vectorized environment (VecEnv), using massively parallel simulation described in Section 4, ensuring a diverse experience and learning exposure. We introduce dataset noise and KL divergence penalty to increase diversity.
%     \item \textbf{Validation}. After training, agents are validated with a separate validation environment. We discard poorly performing agents that learned degenerate strategies due to KL divergence penalty or excessive noise.
%     \item \textbf{Weights Calcualtion}. After validation, each agent's performance is quantitatively assessed based on some metrics, such as cumulative returns, Sharpe ratio, or maximum drawdown. These metrics inform the weighting scheme used in the ensemble model for prediction. 
%     \item \textbf{Trading}. A softmax layer is used to consider the importance of each agent’s performance-weighted outputs. The final action is aggregated for prediction in the trading environment.
% \end{enumerate}

% \subsection{Stock Trading Task}
% For the stock trading task, the weights for each agent’s output in the ensemble are determined through a softmax function applied to the Sharpe ratios from validation. As a risk-adjusted return, the Sharpe ratio helps to understand how much return an investment is generating for each unit of risk taken. It is calculated as 
% \begin{equation} \label{sharpe_ratio}
%     \text{Sharpe Ratio} = \frac{\bar{r}_p - r_f}{\sigma_p}
% \end{equation}
% where $\bar{r}_p$ is the expected portfolio return, $r_f$ is a chosen risk-free rate, and $\sigma_p$ is the standard deviation of the portfolio return. Using the Sharpe ratio as a performance metric ensures, and then applying a softmax weight over the shape ratios to weigh the action vectors of agents in the ensemble ensures that the agents with the best balance of returns and risks have a proportionally greater influence on the ensemble decision.

% In addition, our methodology incorporates a rolling window approach for training, validation, and trading:
% \begin{enumerate}
%     \item \textbf{Training}. Each agent is trained within a rolling window with a dataset comprising one month of historical stock market data. This training involves parallel massively simulation within vectorized environments. 
%     \item \textbf{Validation}. Then, agents are separately validated on a rolling window of flexible length. The performance of each agent is assessed based on its ability to maximize the Sharpe Ratio. 
%      \item \textbf{Weights Calcualtion}. Using the agents' Sharpe Ratios, we compute a softmax activation weight for each agent. %Using softmax has the advantage, that all the weights sum to 1 which lets us handle an arbitrary number of agents, it also gives the most weight to the highest values which correspond to better Sharpe Ratios.
%     \item \textbf{Trading}. Each agent in the ensemble is made to predict an action vector over the testing environment. The actions are then scaled by the corresponding weights; the sum of the weighted action vectors is used to trade and predict for the trading window.
% \end{enumerate}
% After each loop, the training, validation, and trading windows are rolled forward such that the agents are always validated and trained on unseen data. This rolling window approach ensures that the ensemble method remains adaptive to the continuously changing market. 



% We perform high-frequency trading (HFT) in the cryptocurrency trading task to take advantage of the high volatility and rapid price movements that are important characteristics of the cryptocurrency market. HFT utilizes sophisticated algorithms designed to make quick decisions based on market data. In the context of our ensemble method for cryptocurrency trading, each agent within the ensemble executes trades at speeds that are crucial in exploiting market inefficiencies.

% The ensemble method utilizes a softmax function on the cumulative returns of these agents to determine their respective weights in the final decision-making process. The steps are as follows:
% \begin{enumerate}
%     \item \textbf{Training}. Each agent within the ensemble is independently trained using historical cryptocurrency market data with massively parallel simulation. This data includes various market conditions with frequency in seconds, aiming to equip each agent with robust trading strategies suitable for high-frequency operations. 
%     \item \textbf{Validation}. Agents separately interact with the validation environment. This process assesses each agent's ability to generate profitable returns over short periods within the high-frequency trading context. 
%     \item \textbf{Weights Calcualtion}. The weights for each agent's influence on the ensemble decision are assigned based on the results of softmax on their cumulative returns from the validation phase.
%     \item \textbf{Trading}. The final trading action taken by the ensemble is a weighted aggregate of the outputs of all agents.
% \end{enumerate}

% The ensemble method for high-frequency crypto trading effectively harnesses the collective capabilities of multiple specialized agents, each contributing to a unified decision-making process. 


% The ensemble comprised four instances of Proximal Policy Optimization (PPO) and three instances of Soft Actor-Critic (SAC). These models were trained independently on the in-sample data to develop distinct trading strategies. Post-training, agents were validated based on their ability to generate cumulative returns. Weights for each agent’s outputs in the ensemble were assigned using a softmax function applied to the cumulative returns obtained during this validation phase. 

%In this paper, we investigated two significant challenges of financial reinforcement learning, policy instability and the sampling bottleneck. By integrating ensemble method with massively parallel simulations on GPUs, we enhanced both the efficiency and robustness of trained models in volatile financial markets. Our massively parallel simulations substantially improved the sampling speed by $\times$ using $2048$ parallel environments, which facilitates the experience replay of extensive financial datasets for robust ensemble models. The ensemble methods leverage the strengths of multiple diverse agents, which not only improves overall profitability but also diversifies risk. Our experiments on both stock trading and cryptocurrency trading tasks demonstrated that the ensemble method consistently outperforms individual models in terms of returns and risk management. 

==> sections/introduction.tex <==
Advancements in reinforcement learning (RL) have led to significant breakthroughs across various domains, notably in financial markets where decision-making is crucial. Financial reinforcement learning focuses on applying RL techniques to financial tasks, where developing trading strategies remains a primary emphasis. Given the complexity and high computational demands of these tasks, efficient and robust solutions are essential. 

However, two major challenges significantly impact the efficiency and reliability of models: the sampling speed bottleneck and policy instability. The bottleneck in sampling speed predominantly arises from the intensive computational requirements of simulating complex financial markets, where data sampling is an inherently time-consuming process. The training process involves a simulation phase executed on CPUs, which manages the sequential and detailed data sampling and reward calculation tasks. Following simulation, the learning phase takes place, typically on GPUs, which handle the parallel computations needed for policy updates. The latency involved in transferring data between CPUs and GPUs is another reason for the bottleneck, which hampers the seamless integration of the simulation and learning processes. Another significant challenge is the instability of policies in financial reinforcement learning. Financial markets are inherently complex and dynamic, characterized by high volatility and a low signal-to-noise ratio, which complicates the task of developing stable and reliable strategies. RL models in such settings often exhibit high variance in their performance, leading to inconsistent and sometimes unreliable outcomes.

This paper presents a massively parallel simulation approach and ensemble strategy to address these challenges. First, we develop vectorized environments for both stock and cryptocurrency trading tasks, allowing for the execution of several thousand parallel market environments on a single GPU. This approach significantly enhances the speed and efficiency of simulations. Second, we implement an ensemble strategy to enhance the stability and reliability of the learned policies. By weighted averaging the outputs of multiple agents, we reduce the variance and improve the overall performance.

Following this introduction, the structure of the paper is organized as follows: Section 2 reviews related works. Section 3 gives the description of the trading problem. Section 4 delves into the implementation of the vectorized environments and the setup of massively parallel simulations on GPUs. Section 5 describes the ensemble strategy in detail, including the model selection and weighting criteria. Section 6 describes the experimental setup and presents the results, with a comparative analysis of performance across various settings and scenarios. The paper concludes with Section 7, summarizing the findings and implications of the study.


==> sections/related.tex <==
\subsection{Financial Reinforcement Learning}
In recent years, RL techniques have successfully solved sophisticated decision-making environments, beating human experts at challenging games and tasks such as Go, Chess, and StarCraft m\cite{silver2018general} \cite{6637024}. These impressive results demonstrate the inherent strength of RL techniques when applied to complex environments that have low signal-to-noise ratios and very large action spaces. In addition to their successes in game and robotics environments, RL techniques have also proven effective in solving complicated and noisy financial problems such as stock or futures trading \cite{10.1145/3490354.3494366}. This demonstrates that there is a strong academic backing for the effectiveness of RL techniques in complex environments especially trading assets on financial markets.

\subsection{GPU-based Simulation Environments}
RL algorithms rely heavily on simulated environments for training, especially financial algorithms need to be trained and verified on historical data before being deployed to real-world applications. To date, market simulation environments leverage CPUs to run the environments, whilst the models are trained on GPUs \cite{10.1145/3384441.3395986}. These pipelines limit the number of environments to the number of CPU cores and introduce latency when information is passed between the CPU and GPU. This is a large bottleneck in financial settings, where data is simple and frequently updated.  In recent years GPU-based simulation environments have demonstrated their ability to exponentially increase the number of environments and the sampling rate of RL algorithms at higher computational efficiency \cite{makoviychuk2021isaac}.

\subsection{Ensemble Learning}
Ensemble learning methods combine the predictions of multiple learning algorithms to obtain better performance than the individual parts \cite{https://doi.org/10.1002/widm.1249}. Due to the complex nature of financial environments and the distinct qualities of different predictive algorithms, ensemble learning methods can provide enhancements in policy stability and predictive power, especially when adjusted to certain criteria such as risk or final returns \cite{yang2020deep}. 

==> sections/vecenv.tex <==
% IV. Vectorized Env (name is to be changed) (Nik)
%     1. stock trading vec env
%         i. env: reset, step, reward (using vmap)
%     2. crypto trading vec env

Our vectorized stock trading environments seek to solve the issue of sample loading latency, as well as the sampling rate of the agent in the environment.  

We present a vectorized stock trading environment that enables simulating markets and training models exclusively on the GPU. By doing this we are able to increase the sampling speed since we remove the latency of GPU-CPU communication, and we are able to increase the sampling rate by running thousands of simulations in parallel. We follow the design paradigms of other vectorized simulation environments ~\cite{makoviychuk2021isaac}. In the vectorized environment, we adapt the MDP from the unvectorized problem statement ~\cite{liu2024dynamic} by adding a new dimension representing the number of environments to the observation and action spaces as shown in Figure \ref{fig:producer_consumer}. We vectorize key steps of the MDP described earlier to create \texttt{StockTradingVecEnv}, a vectorized gym-style stock trading environment.

The \texttt{StockTradingVecEnv} is controlled by the functions \texttt{reset(), step(), reward()} which behave in a vectorized manner, operating on all rows of the state matrix in parallel. We make use of PyTorch's \texttt{torch.vmap()} to vectorize the functions.


\begin{itemize}
    \item \texttt{reset()}: $s_t \rightarrow s_0$ sets each state tensor in the state matrix to the user-defined default state.
    \item \texttt{step()}: $s_t \rightarrow s_{t+1}$ changes the state in each environment in parallel.
    \item \texttt{reward()}: $(s_t, a_t, s_{t+1}) \rightarrow r_t$ for all environment tensors the rewards for a high dimensional action are computed in parallel. 
\end{itemize}

In this vectorized stock trading environment we are able to determine the per-step sample rate from the dimensions of the environment. At each time step, we observe $N$ different stocks in $E$ different environments. An exponentially higher number of environments therefore leads to an exponentially higher sampling rate at similar compute times. 
